Survey of Gravitationally lensed Objects in HSC Imaging (SuGOHI) -- VII. Discovery and Confirmation of Three Strongly Lensed Quasars

We present spectroscopic confirmation of three new two-image gravitationally lensed quasars, compiled from existing strong lens and X-ray catalogs. Images of HSC J091843.27$-$022007.5 show a red galaxy with two blue point sources at either side, separated by 2.26 arcsec. This system has a source and a lens redshifts $z_s=0.804$ and $z_{\ell}=0.459$, respectively, as obtained by our follow-up spectroscopic data. CXCO J100201.50$+$020330.0 shows two point sources separated by 0.85 arcsec on either side of an early-type galaxy. The follow-up spectroscopic data confirm the fainter quasar has the same redshift with the brighter quasar from the SDSS fiber spectrum at $z_s=2.016$. The deflecting foreground galaxy is a typical early-type galaxy at a redshift of $z_{\ell}=0.439$. SDSS J135944.21$+$012809.8 has two point sources with quasar spectra at the same redshift $z_s=1.096$, separated by 1.05 arcsec, and fits to the HSC images confirm the presence of a galaxy between these. These discoveries demonstrate the power of the Hyper Suprime-Cam Subaru Strategic Program (HSC-SSP)'s deep imaging and wide sky coverage. Combined with existing X-ray source catalogues and follow-up spectroscopy, the HSC-SSP provides us unique opportunities to find multiple-image quasars lensed by a foreground galaxy.

==> 2020_SuGOHI_VII%20(MNRAS-A)/macros.tex <==
% References:
\newcommand{\aref}[1]{Appendix~\ref{#1}}
\newcommand{\sref}[1]{Section~\ref{#1}}
\newcommand{\fref}[1]{Figure~\ref{#1}}
\newcommand{\fsref}[1]{Figures~\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\eref}[1]{Equation~(\ref{#1})}

% LENSING 
\def\zcl{z_{\rm cl}}
\def\zl{z_{\ell}}
\def\zls{z_{\ell,\rm spec}}
\def\zlp{z_{\ell,\rm phot}}
\def\zs{z_{\rm s}}
\def\Rarc{R_{\rm arc}}
\def\MEin{M_{\rm Ein}}

\newcommand{\ant}[1]{\textcolor{magenta}{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
